Guided Generative Adversarial Neural Network for Representation Learning and High Fidelity Audio Generation using Fewer Labelled Audio Data

Recent improvements in Generative Adversarial Neural Networks (GANs) have shown their ability to generate higher quality samples as well as to learn good representations for transfer learning. Most of the representation learning methods based on GANs learn representations ignoring their post-use scenario, which can lead to increased generalisation ability. However, the model can become redundant if it is intended for a specific task. For example, assume we have a vast unlabelled audio dataset, and we want to learn a representation from this dataset so that it can be used to improve the emotion recognition performance of a small labelled audio dataset. During the representation learning training, if the model does not know the post emotion recognition task, it can completely ignore emotion-related characteristics in the learnt representation. This is a fundamental challenge for any unsupervised representation learning model. In this paper, we aim to address this challenge by proposing a novel GAN framework: Guided Generative Neural Network (GGAN), which guides a GAN to focus on learning desired representations and generating superior quality samples for audio data leveraging fewer labelled samples. Experimental results show that using a very small amount of labelled data as guidance, a GGAN learns significantly better representations.

==> abstract.tex <==

\noindent Recent improvements of Generative Adversarial Neural Network (GAN) have shown its capability of generating higher quality samples as well as learning good representation for transfer learning. Most of the representation learning methods with GAN learn representation in a manner ignoring its post-use scenario, which leads to generalisation but increases the redundancy of the model if it is intended to be used for a specific task. Suppose we have a vast unlabelled audio dataset and want to learn representation from this dataset in a way so that it can be used later to improve emotion recognition capability from a fewer labelled audio dataset. During the representation learning training, the model has no idea of the post emotion recognition task, so it can ignore that emotion related characteristics in the learned representation, which will be a failure for this model resulting in the waste of resources for training the model. This is a common problem for any unsupervised representation learning model, and to mitigate this problem, we have proposed a GAN framework named Guided Generative Neural Network (GGAN), which guides GAN to focus on learning desired representation and generating superior quality samples for audio data leveraging fewer labelled samples. As our GGAN is built top on the famous BigGAN architecture, we have explored the impact of the BigGAN architecture on Audio generation in this paper and finally proposed a new model named Guided Generative Neural Network (GGAN) which has performed superior in terms of generation as well as representation learning with guidance from fewer number of labelled samples.            


==> intro_bkp1_1.tex <==
Learning meaningful representation from the unlabelled dataset is a challenging task \cite{goodfellow_book:2016} but recent advancement of the Generative Adversarial Neural Network (GAN) \cite{goodfellow:2014} has shown great success \cite{donahue2019large, dumoulin2016adversarially, DonahueKD16} in this field. Recent work of Deepmind \cite{donahue2019large} shows that the superior generation power of GAN~\cite{karras:2017, karras2019style, Andrew_biggan} is useful for learning good representation. While the successes of the GAN are based on the image generation tasks, it does not perform well on the audio generation tasks \cite{engel2019gansynth}. Encouragingly, recently some studies \cite{engel2019gansynth,chris_wspecgan,andrTIFGAN} have shown intriguing results in audio generation. This prompts for further studies of these methods to learn representation from unlabelled audio data. Now a days disentangled representation is getting tremendous interest as it offers different factor of variations of any dataset to be easily separable in the representation space \cite{bengio2013representation} which is an indication for a good representation learning \cite{peters2017elements,bengio2013representation,goodfellow_book:2016, Michael05069}. Though some GAN based studies have claimed good result for learning disentangled representation from unlabelled data \cite{radford2015,zhao:2017,chen2016infogan,makhzani:2016,chorowski_wavenet_autoencoder,karras2019style,donahue2019large}, recent work of Google AI has shown both theoretically and practically that unsupervised disentangled representation learning is fundamentally impossible and some form of supervision is necessary to achieve this goal \cite{francesco_2019}. Therefore, for learning a good representation using GANs, it requires good generation as well as some supervision.

\noindent Direct generation of the raw audio waveform is a very complex task. The wavenet generative neural network \cite{waveNet} got some success in raw waveform generation, however, the proposed method was computationally expensive and slow. Rather than using GANs to generate a raw waveform, recent works on generating audio spectrogram (time-frequency representations of audio) and then converting them to audio has shown tremendous success \cite{GANSynth08710, chris_wspecgan,marafioti2019adversarial}. In this process, if the spectrogram can be generated successfully, the next challenge becomes to the conversion of the spectrogram to the audio. In TiFGAN paper \cite{marafioti2019adversarial} using the Phase-gradient heap integration (PGHI) \cite{zden_25} method, authors have shown a minimal loss for audio reconstruction from the spectrogram. Among the GAN architectures, the BigGAN model has performed better in terms of image generation and also in terms of representation learning \cite{Andrew_biggan}. So BigGAN can be used to generate a high-quality spectrogram and representation. Nevertheless, to achieve a better result with BigGAN architecture, we need to provide an enormous amount of data with labels \cite{lucic2019highfidelity}. Though it is easy to find lots of open-sourced datasets, getting labels for them is very expensive. However, the recent work of Deepmind with BigGAN has achieved state of the art (SOTA) generation \cite{lucic2019highfidelity} performance using fewer labels, but the methods discussed in the paper are not suitable for representation learning.

\noindent Representation learning from unlabelled data is ideal so that it can be used for other scenarios where vast labels data is not presented. 
Here we learn representation from one dataset and then use it for another dataset, so the validation of the representation learning can not be conducted after the completion of the first training, making representation learning very difficult. Suppose we have a huge amount of unlabelled audio data of different animal sounds along with daily human-made sounds and a small labeled dataset for classifying x numbers of animal sounds. We assume that these specific animal sounds are presented in the unlabelled dataset. Now we want a model to learn representation from this unlabelled audio data disentangling the animal sound characteristics so that it can be used to learn animal sound classification from the small labeled dataset. But recent work of Google AI \cite{francesco_2019} has claimed that perfect disentangled representation can not be learned from unsupervised methods, so there is no guarantee that this model will disentangle animal sounds in the representation space making it unreliable for post animal sound classification training. It would be useful if we could guide the model to learn post task specific representation so in this paper, we have tried to address this problem through proposing a new GAN architecture where we can guide the GAN model with small labeled data samples to focus on specific characteristics when learning the representation as well as generates superior quality samples. Our contribution in this paper can be summarized as


\begin{itemize}
\item We have proposed a new guided representation learning model named Guided Generative Adversarial Neural Network (GGAN). The sample generation and representation learning capability is justified.  
\item As our model is based on the BigGAN model, we have explored the bigGAN architecture for generating audio spectrograms in both unsupervised and supervised manner, where we have validated the model after converting the spectrogram to audio. The representation learning of the unsupervised BigGAN is explored for audio data.     
\end{itemize}








==> justbackup.tex <==
% %\documentclass[a4paper,12pt]{article}

% \usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
% \usepackage[utf8]{inputenc}
% \usepackage{sectsty}
% \usepackage{titlesec}
% \usepackage{import}
% \title{
% % High-Quality Audio Generation and Representation Learning with Guided Generative Adversarial Neural Network (GGAN) using Fewer Labelled Data
% % / 
% Guided Generative Adversarial Neural Network for Learning Task-specific Representation and Generating High-Quality Audio Sample Leveraging Fewer Labelled Audio Data
% }
% \author{}
% \date{September 2018}
% \setcounter{secnumdepth}{4}
% \usepackage{graphicx}
% \graphicspath{ {images/} }
% % \documentclass[a4paper,12pt]{article}
% % \usepackage[utf8]{inputenc}
% % \usepackage[english]{babel}
% \usepackage{graphicx}
% % \usepackage[round]{natbib}
% % \usepackage[nottoc]{tocbibind} %Adds "References" to the table of contents
% % For algorithms
% \usepackage{algorithm}
% % \usepackage{algorithmic}
% \usepackage{amsmath}
% \usepackage{algcompatible}
% \usepackage{globalThings}
% % \usepackage[utf8]{inputenc}
% % \usepackage{blindtext}
% % \usepackage[utf8]{inputenc}
% % \usepackage{blindtext}
% \usepackage{color}
% % \import{}{front_page.tex}
% % %Document title, author and date (empty)
% % \title{Unsupervised  Disentangled  Representation Learning  from  audio}
% % \author{Kazi Nazmul Haque}
% % \date{}
% % \usepackage{pageslts}
% % \usepackage{fancyhdr}
% % \pagestyle{fancy} 
% % \fancyhf{}
% % \renewcommand{\headrulewidth}{0pt}
% \usepackage{pageslts}
% \usepackage{fancyhdr}
% \pagestyle{fancy} 
% \fancyhf{}
% \renewcommand{\headrulewidth}{0pt}
% \usepackage{setspace}

% \usepackage{xfrac}
% % \usepackage{lineno}
% \usepackage{longtable}


% \begin{document}

% % \doublespacing
% % % \newpage
% % % \renewcommand*\contentsname{Table of Contents}
% % \pagenumbering{roman}
% % \cfoot{\thepage}
% % \tableofcontents
% % \clearpage

% % \pagenumbering{arabic}
% % \cfoot{\thepage}
% % \linenumbers

% \maketitle

% % \begin{abstract}


% % \import{}{abstract.tex}
 




% % \end{abstract}






% % %\section{Introduction}
% % %\import{}{intro.tex}

% % %\section{Background and Related Work}
% % %\import{}{background.tex}


% % %\section{Proposed Research Methods}

% % %\import{}{proposed_method.tex}

% % \section{Data and Implementation Detail}
% % %\import{}{data.tex}

% % \section{Results}
% % %\import{}{results.tex}

% % \section{Conclusion}
% % %\import{}{conclusion.tex}

% % \newpage
% % \medskip
% % \bibliographystyle{acm}
% % \bibliography{references}



% \end{document}








==> results_old.tex <==
For comparing the result of GGAN model, we have trained unsupervised and supervised BigGAN model on S09 dataset. For GGAN model, we need to validate two tasks, one is the representation learning, and another one is the sample generation quality. During the validation of representation learning, we also need to verify whether pre guidance is useful for representation learning or not. We expect the GGAN model to outperform unsupervised BigGAN in terms of representation learning and sample generation. We also expect the sample generation quality to be similar or nearby to the supervised BigGAN. 


% Before implementing the GGAN model, we have trained unsupervised and supervised BigGAN model on S09 dataset to understand their behaviour as well as for a comparison with GGAN. We had a clear intention to understand whether the representation learned by GGAN is better than any powerful unsupervised GAN, and our GGAN should perform better than any  GAN or near to any supervised GAN. 


\subsection{Unsupervised and Supervised BigGAN}

For unsupervised BigGAN model, we achieved an IS score of 6.17±.2 and an FID score of 24.72 where we received IS score of 7.33±.01 and FID score of 24.40 ± .5 for the supervised BigGAN. Due to having the access to all label information, Supervised BigGAN performed better than the unsupervised BigGAN. But the performance of both networks is better than any other research works showed in the table \ref{tab:my-table}. 


% We have used BigGAN Architecture for the generation of the audio log-magnitude spectrogram for the s09 dataset. For unsupervised BigGAN, we achieved an IS score of 6.17±.2 and an FID score of 24.72 where we received IS score of 7.33±.01 and FID score of 24.40 ± .5 for the supervised setting. As usual, Supervised BigGAN performed better than the unsupervised BigGAN. But the performance of both networks is better than any other research works showed in the table \ref{tab:my-table}. 

\noindent Though we have achieved state of the art sample generation result with the unsupervised BigGAN architecture, we found inconsistency in the latent space.


When we did linear interpolation between two random points in the latent space like the DCGAN paper \cite{radford2015}, we found a smooth transition in the generated spectrogram space but after converting them to the audio, we found the transaction non-smooth. 
\noindent In figure \ref{fig:fig1}, we can observe the generated spectrogram by the generator where the latent input vectors were the result of the linear interpolation between two random latent points. For the first latent point (most left in the figure), the generator has created spectrogram for digit 2 with a male voice, and for the other point (most right in the figure), it has created digit 2 with a female voice. In between are the spectrograms for the interpolated latent vectors. From left to right, we can see a smooth transition between the spectrograms, but when we converted it to the audio form, after the first sample digit 2 with the male voice, we got digit 8 with a new male and female voice. Then there is the digit 2 with the desired female voice. In this example, the digit was the same for two samples (most left and right in the figure), but the voice was changed from male to female. In the audio space, we have noticed the smooth transition for the speaker's voice, but for the digit, we found 8 in between, which is unexpected and shows that the generator was unable to disentangle the information of the digit category properly. 



% In figure \ref{fig:fig2}, we have also noticed the same problem in the interpolation between male voice digit 8 to male voice digit 0. From this, we can understand that the generator was not able to disentangle the major property of the dataset, which is a problem later task such as data augmentation and representation learning. This problem was not found in the supervised BigGAN.      


\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=\textwidth]{images/1.png}}
    \caption{ Generated Spectrogram from the interpolation of the latent space from the male sound of digit 2 to the female sound of digit 2 (left to right). }
    \label{fig:fig1}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=\textwidth]{images/2.png}}
    \caption{ Generated Spectrogram from the interpolation of the latent space from the male sound of digit 8 to the male sound of digit 0 (left to right). }
    \label{fig:fig2}
\end{figure*}


For learning the representation for the real data samples, we implemented the strategy from the Adversarially learned inference paper \cite{dumoulin2016adversarially} and trained a feature extraction layer top of the trained discriminator network. To evaluate the representation, we have trained a classifier for the digit recognition with a fewer label such as 1 to 5 percent and table \ref{tab:my-table2} show us the result.  


% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{table}
\centering
\caption{Comparison of the performance of the audio generation for different research works}
\label{tab:my-table}
\begin{tabular}{|l|l|l|}\hline
\textbf{Model Name} & \textbf{IS Score} & \textbf{FID Score} \\ \hline
Real (Train) & 9.18 ± 0.04 & - \\ \hline
Real (Test) & 8.01 ± 0.24 &  -\\ \hline
TiFGAN & 5.97 & 26.7 \\ \hline
WaveGAN & 4.67 ± 0.01 &  -\\ \hline
SpecGAN & 6.03 ± 0.04 &  -\\ \hline
Supervised BigGAN & 7.33±.01 & 24.40 ± .5  \\ \hline
Unsupervised BigGAN & 6.17±.2 & 24.72±.05 \\ \hline
GGAN & 7.24±.05 & 25.75±.1 \\ \hline
\end{tabular}
\end{table}


\subsection{GuidedGAN (GGAN)}

\noindent We have implemented our GGAN model with the S09 dataset and achieved IS score of 7.24±.05  and FID score of 25.75±.1 for audio samples using the guidance from 5 percent label data, which is almost near to the performance of the fully supervised Biggan model and far more better than unsupervised BigGAN. 

\begin{figure*}[h]
    \centering
    \frame{\includegraphics[width=\textwidth]{audios.png}}
    \caption{ Generated log-magnitude spectrograms for different conditions. The rows represents different samples generated for different latent space for the given condition (digits)}
    \label{fig:fig3}
\end{figure*}


\noindent GGAN model not only performed Superior in terms of generation but also performed state of the art in the representation learning. With 5 percent label data, we have achieved approximately the test classification accuracy of 95. If we compare the result from table \ref{tab:my-table2} for GGAN and Unsupervised GAN, we can see that for a similar number of the labeled dataset, we have achieved better results with the GGAN. At the same time, it also performed better at generation. 

\begin{table}
\centering
\caption{Comparison of the test accuracy for unsupervised GAN and GGAN}
\label{tab:my-table2}\\
\begin{tabular}{|l|l|l|}\hline
\textbf{Training Data Size} & \textbf{Unsupervised GAN} & \textbf{GGAN} \\ \hline
1\% & 73 ± 1.02 &  84 ± 2.24\\ \hline
2\%  & 75 ± 0.41 &  85 ± 1.24\\ \hline
3\%  & 78 ± 0.07 & 88 ±.1 \\ \hline
4\%  & 80 ± 0.01 &  92 ± 0.5 \\ \hline
5\%  & 80 ± 1.72 &  94 ± 1.2\\ \hline
\end{tabular}
\end{table}

\noindent We have also use TSNE to visualize the learned representation space for the test dataset. Figure \ref{fig:fig3} shows the representations, and we can see that the learned representations are easily classifiable.


\begin{figure}[h]
    \centering
    \frame{\includegraphics[width=.8\linewidth]{images/embfinal.png}}
    \caption{ TSNE visualisation of the learned embedding on the test dataset. }
    \label{fig:fig3}
\end{figure}

\noindent For the second experiment, we have achieved generated samples of S09 for males and females for two different conditions. So the guidance of gender has worked successfully from a completely different dataset. We achieved IS score of 6.52 ± .5 and FID score of 26.21 ± .1. Though our GGAN model was not guided for digit categories, it has SOTA performance. 



\noindent Among many minor challenges, the main challenge we faced was related to the generation of the model. There was a severe issue of mode collapse, which we could not fix implementing different techniques in the literature \cite{salimans:2016}. So we got inspiration from the Mode Seeking GAN \cite{Qi05628} work and modified the loss function and created a unique feature loss, which immediately fixed the mode collapse problem. The feature loss calculates the ratio of the difference between the two real samples and two generated samples. The whole model wants to minimise this loss until the value one. If the generator creates very similar or the same sample, then it gets penalised and tries to find more modes.  In the supplement material section, we have provided the detail of the training and the discussion on the behaviour of the losses as these are an essential guideline for reproducing the results or improve the work only.



==> texes/metadaten.tex <==
%%Hier alle Daten einfügen
\newcommand{\autorname}{Kazi Nazmul Haque (u1104280)}

\newcommand{\Program}{Doctor of Philosophy (DPHD)}
\newcommand{\Faculty}{Faculty of Health, Engineering, and Sciences}
\newcommand{\School}{Agricultural, Computation and Environment Science}
\newcommand{\ps}{Dr Rajib Rana}
\newcommand{\as}{Ji Zhang}
\newcommand{\lp}{Lehrperson}
\newcommand{\arbtyp}{}
\newcommand{\titel}{Learning Unsupervised Distangled Representation
From Audio for Transfer Learning.}
\title{\titel}
\author{\autorname}








% Program: 
% Faculty: 
% School: School of Psychology and Counselling
% Area of study: Health Systems and Behaviour
% Principal Supervisor: Assoc. Prof. Sonja March
% Associate Supervisors: Dr. Belinda Goodwin, Prof. Jeff Dunn AO

==> texes/titlepage.tex <==
\begin{titlepage}
\vspace*{4cm}
\begin{tabu} to \textwidth {X[c]}
	\toprule
	\toprule[2pt]
	\huge{\textsc{\titel}}\\
	\Large{\textsc{\arbtyp}}\\
	\bottomrule[2pt]
	\bottomrule
\end{tabu}
\\[3cm]
\centering{
\textsc{\Large \autorname}
}
\\[3cm]
\begin{tabu} {>{\itshape}X[r] X[1.5]}
Program & \Program\\
Faculty & \Faculty\\
School & \School\\
Principle Supervisor & \ps\\
Associate Supervisors & \as \\
\end{tabu}
\vfill
\includegraphics[width=3cm]{res/usq.jpg}

\end{titlepage}

